Taming Normalizing Flows

We propose an algorithm for taming Normalizing Flow models - changing the probability that the model will produce a specific image or image category. We focus on Normalizing Flows because they can calculate the exact generation probability likelihood for a given image. We demonstrate taming using models that generate human faces, a subdomain with many interesting privacy and bias considerations. Our method can be used in the context of privacy, e.g., removing a specific person from the output of a model, and also in the context of debiasing by forcing a model to output specific image categories according to a given target distribution. Taming is achieved with a fast fine-tuning process without retraining the model from scratch, achieving the goal in a matter of minutes. We evaluate our method qualitatively and quantitatively, showing that the generation quality remains intact, while the desired changes are applied.

==> figs/ablation_distribution.tex <==
\begin{figure}[t]
    \centering
    
    \includegraphics[width=\linewidth,keepaspectratio]{images/ablation_distribution.pdf}

    \caption{}
    \label{fig:ablation_distribution}
\end{figure}
